A Universal Primal-Dual Convex Optimization Framework

We propose a new primal-dual algorithmic framework for a prototypical constrained convex optimization template. The algorithmic instances of our framework are universal since they can automatically adapt to the unknown Holder continuity degree and constant within the dual formulation. They are also guaran- teed to have optimal convergence rates in the objective residual and the feasibility gap for each Holder smoothness degree. In contrast to existing primal-dual algorithms, our framework avoids the proximity operator of the objective function. We instead leverage computationally cheaper, Fenchel-type operators, which are the main workhorses of the generalized conditional gradient (GCG)-type methods. In contrast to the GCG-type methods, our framework does not require the objective function to be differentiable, and can also process additional general linear inclusion constraints, while guarantees the convergence rate on the primal problem

==> PDUGA_impl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 4. Modifications and extensions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-2ex}
\section{Frank-Wolfe's algorithm is dual averaging}\label{sec:related2FW}
\vspace{-1ex}
The universal gradient method covers subgradient algorithms as special cases when $\nu = 0$.
In this section, we show  that the Frank-Wolfe (FW) algorithm overviewed in \cite{Jaggi2013} is can be cast as a variant of the dual averaging subgradient algorithm \cite{Nesterov2009b} with an appropriate choice of the proximity function.

The Frank-Wolfe algorithm as revisited in \cite{Jaggi2013}  aims at solving the following constrained convex problem:
\begin{equation}\label{eq:constr_cvx2}
\vspace{-0.5ex}
\varphi^{\star} := \min_{\xb}\set{ \varphi(\xb) : \xb\in \Xc},
\vspace{-0.25ex}
\end{equation}
where $\Xc$ is a nonempty, closed, convex and bounded, and $\varphi$ is a smooth convex function (with Lipschitz gradient).
The FW algorithm generates a sequence $\{\bar{\xb}_k\}$ using:
\begin{equation}\label{eq:FW_alg}
\vspace{-0.5ex}
\left\{\begin{array}{ll}
\hat{\xb}_{k+1} &:= \arg\displaystyle\min_{\xb}\{\iprods{\nabla{\varphi}(\xbar_k), \xb} : \xb \in\Xc\}\\
\bar{\xb}_{k+1} &:= \bar{\xb}_k + \gamma_k(\hat{\xb}_{k+1} - \bar{\xb}_k),
\end{array}\right.
\vspace{-0.25ex}
\end{equation}
where $\gamma_k\in (0, 1]$ is the step-size. 
We can either set $\gamma_k := \frac{2}{k+2}$ or determine it via a line-search procedure.

Let us introduce $\rb := \xb$. Then we can rewrite \eqref{eq:constr_cvx2} as  \eqref{eq:constr_cvx}:
\begin{equation}\label{eq:constr_cvx2b}
\vspace{-0.5ex}
\varphi^{\star} = \min_{\xb, \rb}\set{\varphi(\rb) : \xb - \rb = 0, ~\xb\in\Xc}.
\vspace{-0.25ex}
\end{equation} 
The dual function \eqref{eq:dual_composite} for \eqref{eq:constr_cvx2b} is then given by 
\begin{equation*}
\vspace{-0.5ex}
G(\lbd) := \varphi^{*}(\lbd) + \sup_{\xb\in\Xc}\iprods{-\lbd,\xb},
\vspace{-0.25ex}
\end{equation*}
where $\varphi^{*}$ is the Fenchel conjugate of $\varphi$ and $s_{\Xc}$ is the support function of $\Xc$.
By definition, we can estimate
\begin{equation*}
\vspace{-0.5ex}
\nabla{G}(\lbd) =\nabla{\varphi^{*}}(\lbd) -\xopt(\lbd),  ~\xopt(\lbd) := \mathrm{arg}\!\min_{\xb\in\Xc}\iprods{\lbd, \xb}.
\vspace{-0.25ex}
\end{equation*} 
If we define $\bar{\xb}_k := \nabla{\varphi^{*}}(\bar{\lbd}_k)$, then $\bar{\lbd}_k = \nabla{\varphi}(\bar{\xb}_k)$.
Let $\hat{\xb}_{k+1} := \xopt(\bar{\lbd}_k)$, then $\hat{\xb}_{k+1} = \xopt(\nabla{\varphi}(\bar{\xb}_k))$.
Hence, $\nabla{G}(\bar{\lbd}_k) := -(\hat{\xb}_{k+1} - \bar{\xb}_k)$.
Using these expressions, we can equivalently reformulate \eqref{eq:FW_alg} as:
\begin{equation}\label{eq:dual_update}
\vspace{-0.5ex}
\text{Frank-Wolfe}: \left\{\begin{array}{ll}
\bar{\xb}_{k\!+\!1} &:= \bar{\xb}_k \!-\! \gamma_k\nabla{G}(\bar{\lbd}_k)\\
\bar{\lbd}_{k+1} &:= \nabla{\varphi}(\bar{\xb}_{k+1}).
\end{array}\right.
\vspace{-0.25ex}
\end{equation}
Since $\nabla{\varphi}$ is Lipschitz continuous with a Lipschitz constant $L_{\varphi} > 0$, by Baillon-Haddad's theorem \cite{Bauschke2011}, the conjugate $\varphi^{*}$ is strongly convex with the convexity parameter $\mu_{\varphi^{*}} := L_{\varphi}^{-1}$. Hence, we can use $\varphi^{*}$ to define the following mapping:
\begin{equation*} 
\vspace{-0.5ex}
\pi_{\beta}(\sb) = \argmin_{\lbd}\set{\iprods{-\sb,\lbd} + \beta \varphi^{*}(\lbd)},
\vspace{-0.25ex}
\end{equation*}
in order to map the primal variable $\xb$ to the dual variable $\lbd$. 
Using $\pi_{\beta}$, we can easily obtain that:
\begin{equation*} 
\vspace{-0.5ex}
\bar{\lbd}_{k+1} = \pi_{1}(-\xbar_{k+1}), 
\vspace{-0.25ex}
\end{equation*} 
and hence \eqref{eq:dual_update} is exactly cast into the  dual averaging subgradient algorithm for solving the dual problem of \eqref{eq:constr_cvx2b}.
Following \cite{Nesterov2007a,Nesterov2009b}, we can prove that, if $\nabla{G}$ is bounded, then one can show that the convergence rate of $G(\lbd_k) - G^{\star}$ is $\mathcal{O}(1/\sqrt{k})$. If $\nabla{G}$ is Lipschitz continuous, then the convergence rate of $G(\lbd_k) - G^{\star}$ increases to $\mathcal{O}(1/k)$.
The details of this algorithm can be found in the supplementary document. 


==> PDUGA_refs.tex <==
\newpage
{\small
\begin{thebibliography}{10}

\bibitem{Bauschke2011}
H.H. Bauschke and P.~Combettes.
\newblock {\em Convex analysis and monotone operators theory in {H}ilbert
  spaces}.
\newblock Springer-Verlag, 2011.

\bibitem{Beck2009}
A.~Beck and M.~Teboulle.
\newblock {A} {F}ast {I}terative {S}hrinkage-{T}hresholding {A}lgorithm for
  {L}inear {I}nverse {P}roblems.
\newblock {\em SIAM J. Imaging Sciences}, 2(1):183--202, 2009.

\bibitem{Brand2006}
M.~Brand.
\newblock {F}ast {L}ow {R}ank {M}odifications of the thin {S}ingular {V}alue {D}ecomposition.
\newblock {\em Linear Algebra and its Application}, 415:20--30, 2006.

\bibitem{Boyd2011}
S.~Boyd, N.~Parikh, E.~Chu, B.~Peleato, and J.~Eckstein.
\newblock {D}istributed {O}ptimization and {S}tatistical {L}earning via the {A}lternating
  {D}irection {M}ethod of {M}ultipliers.
\newblock {\em Foundations and Trends in Machine Learning}, 3(1):1--122, 2011.

\bibitem{Candes2012b}
E.~Cand\`{e}s and B.~Recht.
\newblock Exact matrix completion via convex optimization.
\newblock {\em Communications of the ACM}, 55(6):111--119, 2012.

\bibitem{Cevher2014}
V.~Cevher, S.~Becker, and M.~Schmidt.
\newblock Convex optimization for big data: Scalable, randomized, and parallel
  algorithms for big data analytics.
\newblock {\em IEEE Signal Processing Magazine}, 31(5):32--43, 2014.

\bibitem{Combettes2008}
P.~L. Combettes and J.-C. Pesquet.
\newblock A proximal decomposition method for solving convex variational
  inverse problems.
\newblock {\em Inverse Problems}, 24(6):065014, 2008.

\bibitem{Goldstein2013}
T.~Goldstein, E.~Esser, and R.~Baraniuk.
\newblock Adaptive {P}rimal-{D}ual {H}ybrid {G}radient {M}ethods for {S}addle
  {P}oint {P}roblems.
\newblock {\em Tech. Report.}, http://arxiv.org/pdf/1305.0546v1.pdf:1--26,
  2013.

\bibitem{Gross2010}
D.~Gross, Y.-K. Liu, S.~T. Flammia, S.~Becker, and J.~Eisert.
\newblock Quantum state tomography via compressed sensing.
\newblock {\em Physical Review Letters}, 105(15):150401(0--4), 2010.

\bibitem{Jaggi2010}
M.~Jaggi and M.~Sulovsk{\'y}.
\newblock {A} {S}imple {A}lgorithm for {N}uclear {N}orm {R}egularized {P}roblems.
\newblock {\em Proceedings of the 27th International Conference on Machine Learning}, 2010.

\bibitem{Jaggi2013}
M.~Jaggi.
\newblock {R}evisiting {F}rank-{W}olfe: {P}rojection-{F}ree {S}parse {C}onvex
  {O}ptimization.
\newblock {\em JMLR W\&CP}, 28(1):427--435, 2013.

\bibitem{Juditsky2013a}
A.~Juditsky and A.~Nemirovski.
\newblock Solving variational inequalities with monotone operators on domains
  given by linear minimization oracles.
\newblock {\em Tech. Report.}, http://arxiv.org/abs/1312.1073, 2013.

\bibitem{Lan2013b}
G.~Lan and R.D.C. Monteiro.
\newblock {I}teration-{C}omplexity of {F}irst-{O}rder {A}ugmented {L}agrangian {M}ethods
  for {C}onvex {P}rogramming.
\newblock {\em Math. Program.}, 2013 (under revision).

\bibitem{Nemirovskii1983}
A.~Nemirovskii and D.~Yudin.
\newblock {\em {P}roblem {C}omplexity and {M}ethod {E}fficiency in
  {O}ptimization}.
\newblock Wiley Interscience, 1983.

\bibitem{Nesterov2005c}
Y.~Nesterov.
\newblock Smooth minimization of non-smooth functions.
\newblock {\em Math. Program.}, 103(1):127--152, 2005.

\bibitem{Nesterov2007a}
Y.~Nesterov.
\newblock Dual extrapolation and its applications to solving variational
  inequalities and related problems.
\newblock {\em Math. Program.}, 109(2--3):319--344, 2007.

\bibitem{Nesterov2009b}
Y.~Nesterov.
\newblock Primal-dual subgradient methods for convex problems.
\newblock {\em Math. Program.}, 120(1, Ser. B):221--259, 2009.

\bibitem{Nesterov2014}
Y.~Nesterov.
\newblock Universal gradient methods for convex optimization problems.
\newblock {\em Math. Program.}, xx:1--24, 2014.

\bibitem{Nesterov2015}
Y.~Nesterov.
\newblock Complexity bounds for primal-dual methods minimizing the model of
  objective function.
\newblock Technical report, Universit{\'e} catholique de Louvain, Center for
  Operations Research and Econometrics (CORE), 2015.

\bibitem{Rockafellar1970}
R.~T. Rockafellar.
\newblock {\em {C}onvex {A}nalysis}, volume~28 of {\em Princeton Mathematics
  Series}.
\newblock Princeton University Press, 1970.

\bibitem{Shefi2014}
R.~Shefi and M.~Teboulle.
\newblock {R}ate of {C}onvergence {A}nalysis of {D}ecomposition {M}ethods
  {B}ased on the {P}roximal {M}ethod of {M}ultipliers for {C}onvex
  {M}inimization.
\newblock {\em SIAM J. Optim.}, 24(1):269--297, 2014.

\bibitem{TranDinh2014b}
Q.~Tran-Dinh and V.~Cevher.
\newblock Constrained convex minimization via model-based excessive gap.
\newblock In {\em Proc. the Neural Information Processing Systems Foundation
  conference (NIPS2014)}, pages 1--9, Montreal, Canada, December 2014.

\bibitem{Wainwright2014}
M.~J. Wainwright.
\newblock Structured regularizers for high-dimensional problems: {S}tatistical
  and computational issues.
\newblock {\em Annual Review of Statistics and its Applications}, 1:233--253,
  2014.

\bibitem{Yu2014}
Yaoliang Yu.
\newblock  {F}ast {G}radient {A}lgorithms for {S}tructured {S}parsity.
\newblock PhD thesis, University of Alberta, 2014.


\end{thebibliography}
}
